A Unified Framework for Multi-Sensor HDR Video Reconstruction

One of the most successful approaches to modern high quality HDR-video capture is to use camera setups with multiple sensors imaging the scene through a common optical system. However, such systems pose several challenges for HDR reconstruction algorithms. Previous reconstruction techniques have considered debayering, denoising, resampling (align- ment) and exposure fusion as separate problems. In contrast, in this paper we present a unifying approach, performing HDR assembly directly from raw sensor data. Our framework includes a camera noise model adapted to HDR video and an algorithm for spatially adaptive HDR reconstruction based on fitting of local polynomial approximations to observed sensor data. The method is easy to implement and allows reconstruction to an arbitrary resolution and output mapping. We present an implementation in CUDA and show real-time performance for an experimental 4 Mpixel multi-sensor HDR video system. We further show that our algorithm has clear advantages over existing methods, both in terms of flexibility and reconstruction quality.

==> macros.tex <==
%
% macros.tex
%

\newcommand{\Var}[1]{\operatorname{Var}\left[#1\right]}

\usepackage{color}
\definecolor{turquoise}{cmyk}{0.65,0,0.1,0.1}
%\usepackage{mathptmx}
\usepackage{graphics,graphicx}
%\usepackage[intlimits]{amsmath}
%\usepackage{amsfonts}
%\usepackage[mathscr]{eucal}
%\usepackage{amsfonts,amssymb,euscript,mathrsfs,bbm}
%\usepackage{epsf,epsfig,wrapfig}
%\usepackage{latexsym}
\usepackage{theorem}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{ctable}
\usepackage{times}
\usepackage{subfig}

%\DeclareGraphicsExtensions{.ps}
% General Commands
\newcommand{\ednote}[1]{{\color{red}[[XXX #1 ]]}} %colour in .ps or pdf only
\newcommand{\todo}[1]{{\color{blue}[[XXX #1 ]]}} %colour in .ps or pdf only
%\newcommand{\etal}{\textit{et al.}}
\newcommand{\namecite}[1]{{\cite{#1}}}
\newcommand{\defn}[1]{\emph{#1}}
\newcommand{\rv}{random variable}
\newcommand{\pdf}{p.d.f.}
\newcommand{\textindegrees}[1]{$#1\,^{\circ}$}

% Math Commands
\newcommand{\mat}[1] {\bs{#1}} %{#1}
\newcommand{\vect}[1]{\bs{#1}}
\newcommand{\uvect}[1]{\bs{\hat{#1}}}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\transp}[1]{{#1}^\mathsf{T}}
\newcommand{\invtransp}[1]{{#1}^\mathsf{-T}}
\newcommand{\inv}[1]{{#1}^{-1}}
\newcommand{\scprod}[2]{#1\cdot#2}
\newcommand{\inprod}[2]{\left<#1,#2\right>}
\newcommand{\reel}{\mathbb{R}}
\newcommand{\rthree}{\reel^3}
\newcommand{\cmplx}{\mathbb{C}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\conj}[1]{\overline{#1}}

% probabiltiy stuff
%\DeclareMathOperator{\pr}{Pr}
\newcommand{\prob}[1]{\pr[#1]}
%\DeclareMathOperator{\expct}{E}
\newcommand{\expect}[1]{\expct[#1]}
\newcommand{\rvX}{X}
\newcommand{\rvXval}{x}
\newcommand{\rvXvct}{\vect{X}}
\newcommand{\rvXvctVal}{\vect{x}}
\newcommand{\pdfX}{f_\rvX}
\newcommand{\covMat}{K}
\newcommand{\covMatX}{K_{\rvX}}
\newcommand{\covMatXvct}{K_{\rvXvct}}
\newcommand{\normX}{\mu_{\rvX}}
%\newcommand{\estNormXvct}{\vect{\mu}_{\rvXvct}}
\newcommand{\estNormXvct}{\vect{\normX}}

% relating to images
\newcommand{\idxs}{\vect{s}}
\newcommand{\nbrs}{\mathcal{N}_{\idxs}}
\newcommand{\nbr}{\mathcal{N}}
\newcommand{\idxr}{\vect{r}}
\newcommand{\idxq}{\vect{q}}
\newcommand{\idxSet}{\Lambda}
\newcommand{\imSide}{N}
\newcommand{\imSz}{\imSide\times\imSide}


\newcommand{\SC}[1]{Section~\ref{#1}}
\newcommand{\SCp}[1]{Section~\ref{#1} on page~\pageref{#1}}
\newcommand{\EQ}[1]{\eqref{#1}}
\newcommand{\EQp}[1]{Equation~\ref{#1} on page~\pageref{#1}}
\newcommand{\FG}[1]{Figure~\ref{#1}}
\newcommand{\FGp}[1]{Figure~\ref{#1} on page~\pageref{#1}}
\newcommand{\TA}[1]{Table~\ref{#1}}
\newcommand{\TAp}[1]{Table~\ref{#1} on page~\pageref{#1}}


\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\sincBCC}{sincBCC}
\DeclareMathOperator{\ramp}{\mathcal{R}}
\DeclareMathOperator{\boxx}{\mathcal{B}}
\DeclareMathOperator{\step}{\mathcal{H}} %{Heaviside}
\DeclareMathOperator{\tesseract}{\mathcal{T}}
\DeclareMathOperator{\hatfcn}{\Lambda}
\DeclareMathOperator{\grad}{\nabla}
\newcommand{\Fourier}[1]{\mathcal{F}\{#1\}}
\newcommand{\shah}{{\textstyle \amalg{\kern-4.pt\amalg}}}

%%
%% my own macros
\newcommand{\eig}{4^{1/3}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\dotdot}{,}

% CONTINUOUS FOURIER TRANSFORM
\newcommand{\cft}[5]{\int_{#1}{ #2 e^{-2\pi i \scprod{#3}{#4}} d#5}}
\newcommand{\icft}[5]{\int_{#1}{ #2 e^{2\pi i \scprod{#3}{#4}} d#5}}
\newcommand{\myfig}[2]{\includegraphics[width=#1\columnwidth]{figures/#2.eps}}
\newcommand{\myimg}[3]{\includegraphics[width=#1\columnwidth]{../images/#2/#3.eps}}
\newcommand{\myerrpic}[3]{\includegraphics[width=#1\columnwidth]{../datasets/#2/errpics/#3.eps}}
%\newcommand{\ml4}[2]{\includegraphics[width=#1\columnwidth]{images/ML40/Data_#2}}
%\newcommand{\ml8}[2]{\includegraphics[width=#1\columnwidth]{images/ML80/Data_#2}}


\newcommand{\RD}{{Rhombic Dodecahedron }}
\DeclareMathOperator{\sincRD}{sincRD}
\DeclareMathOperator{\sincH}{sincH}

\newcommand{\ii}{i}

% inner product
\newcommand{\ip}[2]{\langle #1 , #2 \rangle}

%short for \boldsymbol
\newcommand{\bs}[1]{\boldsymbol{#1}}

%abbreviations for scaled and shifted 3D functions
\newcommand{\scf}[2]{#1_{#2}}
\newcommand{\shf}[2]{#1_{\bs{#2}}}
\newcommand{\ssf}[3]{#1_{#2\mathsf{,}\bs{#3}}}

% centered and non-centered B-splines of degree n, and their derivatives
\newcommand{\cbs}[1]{{\beta}^{#1}}
\newcommand{\dcbs}[1]{\acute{\beta}^{#1}}
\newcommand{\ncbs}[1]{{\beta}_{\triangleright}^{#1}}
\newcommand{\dncbs}[1]{\acute{\beta}_{\triangleright}^{#1}}

% Tensor product B-spline
\newcommand{\tpbs}[1]{{B}^{#1}}

% BCC box spline
\newcommand{\bccbs}[1]{{\Xi}^{#1}}


% Dual of a function
%\newcommand{\dual}[1]{{\overset{\circ}{#1}}}
\newcommand{\dual}[1]{{\mathring{#1}}}


%% Some definitions 
\newcommand{\diffdiff}[3]{\frac{\partial^{#3} {#1}}{\partial {#2}^{#3}}}
\newcommand{\diff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dop}{ {\mathcal{D}} }
\newcommand{\set}[1]{ {\matcal{#1}} }
\newcommand{\order}[1] { \left|#1\right| }
\newcommand{\detd}[1] { {\left|det\left(#1\right)\right|^{\frac{1}{d}}} }
\renewcommand{\vec}[1]{\vect{#1}}

\newcommand{\diag}{\mathop{\mathrm{diag}}}


%\renewcommand{\vec}[1]{\mathbf{#1}}
%\newcommand{\mat}[1]{\mathbf{#1}}
%\newcommand{\norm}[1]{ \left\|\mat{#1}\right\| }
%\newtheorem{thm}{Theorem}[section]
%\newtheorem{cor}[thm]{Corollary}
%\newtheorem{lem}[thm]{Lemma}
%\newtheorem{defi}{Definition}[thm]
\renewcommand{\Re}{\mathbb{R}}
\renewcommand{\arraystretch}{1}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\theorembodyfont{\upshape}
\newtheorem{define}{Definition}[theorem]


